The Proxy Step-size Technique for Regularized Optimization on the Sphere Manifold

We give an effective solution to the regularized optimization problem $g (\boldsymbol{x}) + h (\boldsymbol{x})$, where $\boldsymbol{x}$ is constrained on the unit sphere $\Vert \boldsymbol{x} \Vert_2 = 1$. Here $g (\cdot)$ is a smooth cost with Lipschitz continuous gradient within the unit ball $\{\boldsymbol{x} : \Vert \boldsymbol{x} \Vert_2 \le 1 \}$ whereas $h (\cdot)$ is typically non-smooth but convex and absolutely homogeneous, \textit{e.g.,}~norm regularizers and their combinations. Our solution is based on the Riemannian proximal gradient, using an idea we call \textit{proxy step-size} -- a scalar variable which we prove is monotone with respect to the actual step-size within an interval. The proxy step-size exists ubiquitously for convex and absolutely homogeneous $h(\cdot)$, and decides the actual step-size and the tangent update in closed-form, thus the complete proximal gradient iteration. Based on these insights, we design a Riemannian proximal gradient method using the proxy step-size. We prove that our method converges to a critical point, guided by a line-search technique based on the $g(\cdot)$ cost only. The proposed method can be implemented in a couple of lines of code. We show its usefulness by applying nuclear norm, $\ell_1$ norm, and nuclear-spectral norm regularization to three classical computer vision problems. The improvements are consistent and backed by numerical experiments.

==> results/statistics.tex <==
\begin{tabular}{@{}  c | ccccc | ccccc  @{}} 
\toprule 
& \multicolumn{5}{c|}{$e_{dist}$ (pixels)} & \multicolumn{5}{c}{$e_{rep}$ (pixels)} \\ 
\cmidrule(lr){2-6} \cmidrule(lr){7-11} 
 & 8pt & PGS$_5$ & PGS$_{10}$ &  PGS & Gp & 8pt & PGS$_5$ & PGS$_{10}$ & PGS & Gp \\ 
\midrule 
 Chapel(0,1) & 0.386 & 0.380 & \textit{0.380} & \underline{0.379} & \textbf{0.376} & 0.260 & 0.256 & \textit{0.256} & \underline{0.255} & \textbf{0.254} \\ 
 Keble(0,3) & 0.248 & 0.247 & \textit{0.247} & \underline{0.247} & \textbf{0.247} & 0.175 & 0.175 & \textit{0.175} & \underline{0.175} & \textbf{0.175} \\ 
 Desktop(C,D) & 0.574 & 0.336 & \textit{0.303} & \underline{0.288} & \textbf{0.268} & 0.406 & 0.238 & \textit{0.214} & \underline{0.204} & \textbf{0.190} \\ 
 Library(1,3) & 0.428 & 0.409 & \textit{0.405} & \underline{0.405} & \textbf{0.400} & 0.302 & 0.289 & \textit{0.286} & \underline{0.286} & \textbf{0.282} \\ 
 Merton1(1,3) & 0.308 & 0.295 & \textit{0.291} & \underline{0.288} & \textbf{0.277} & 0.217 & 0.209 & \textit{0.205} & \underline{0.203} & \textbf{0.196} \\ 
 Merton2(1,3) & 0.596 & 0.528 & \textit{0.498} & \underline{0.472} & \textbf{0.404} & 0.421 & 0.373 & \textit{0.352} & \underline{0.334} & \textbf{0.286} \\ 
 Arch & 0.304 & 0.299 & \textit{0.299} & \underline{0.299} & \textbf{0.298} & 0.215 & 0.211 & \textit{0.211} & \underline{0.211} & \textbf{0.211} \\ 
 Yard & 0.433 & 0.429 & \textit{0.429} & \underline{0.428} & \textbf{0.426} & 0.306 & 0.303 & \textit{0.303} & \underline{0.302} & \textbf{0.301} \\ 
 Slate & 0.246 & 0.184 & \textit{0.177} & \underline{0.170} & \textbf{0.163} & 0.129 & 0.097 & \textit{0.093} & \underline{0.089} & \textbf{0.085} \\ 
 Ben1 & 0.203 & 0.144 & \textit{0.128} & \underline{0.102} & \textbf{0.101} & 0.142 & 0.101 & \textit{0.089} & \underline{0.071} & \textbf{0.070} \\ 
 Ben2 & 0.139 & 0.086 & \textit{0.063} & \underline{0.050} & \textbf{0.048} & 0.097 & 0.060 & \textit{0.044} & \underline{0.035} & \textbf{0.033} \\ 
\bottomrule 
\end{tabular} 

